Abusive Span Detection for Vietnamese Narrative Texts

Abuse in its various forms, including physical, psychological, verbal, sexual, financial, and cultural, has a negative impact on mental health. However, there are limited studies on applying natural language processing (NLP) in this field in Vietnam. Therefore, we aim to contribute by building a human-annotated Vietnamese dataset for detecting abusive content in Vietnamese narrative texts. We sourced these texts from VnExpress, Vietnam's popular online newspaper, where readers often share stories containing abusive content. Identifying and categorizing abusive spans in these texts posed significant challenges during dataset creation, but it also motivated our research. We experimented with lightweight baseline models by freezing PhoBERT and XLM-RoBERTa and using their hidden states in a BiLSTM to assess the complexity of the dataset. According to our experimental results, PhoBERT outperforms other models in both labeled and unlabeled abusive span detection tasks. These results indicate that it has the potential for future improvements.

==> tabs/mainres_1.tex <==

\aptLtoX[graphic=no,type=html]{
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|l|llllll|llllll|}
\hline
\multirow{3}{*}{\small{\textbf{Decoder~}}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Training\\ Strategy\end{tabular}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Pre-trained\\ Language\\ Model\end{tabular}}}} & \multicolumn{6}{c|}{\textbf{Strict}} & \multicolumn{6}{c|}{\textbf{Relaxed}} \\ \cline{4-15} 
 &  & \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\textbf{Dev}} & \multicolumn{3}{c|}{\textbf{Test}} & \multicolumn{3}{c|}{\textbf{Dev}} & \multicolumn{3}{c|}{\textbf{Test}} \\ \cline{4-15} 
 &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{F}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{F}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{F}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{F}} \\ \hline
\multirow{8}{*}{\textbf{Softmax}} & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Unlabeled\\ Span\\ Detection\end{tabular}}} & $\text{XLM-R}_\text{base}$ & \multicolumn{1}{j|}{22.22} & \multicolumn{1}{j|}{24.49} & \multicolumn{1}{j|}{23.30} & \multicolumn{1}{j|}{26.89} & \multicolumn{1}{j|}{27.31} & \multicolumn{1}{j|}{27.10} & \multicolumn{1}{j|}{88.00} & \multicolumn{1}{j|}{80.30} & \multicolumn{1}{j|}{83.97} & \multicolumn{1}{j|}{89.00} & \multicolumn{1}{j|}{82.96} & \multicolumn{1}{j|}{85.88} \\ \cline{3-15} 
 &  & $\text{XLM-R}_\text{large}$ & \multicolumn{1}{j|}{20.49} & \multicolumn{1}{j|}{25.51} & \multicolumn{1}{j|}{22.73} & \multicolumn{1}{j|}{24.54} & \multicolumn{1}{j|}{30.77} & \multicolumn{1}{j|}{27.30} & \multicolumn{1}{j|}{85.98} & \multicolumn{1}{j|}{73.93} & \multicolumn{1}{j|}{79.50} & \multicolumn{1}{j|}{80.54} & \multicolumn{1}{j|}{80.79} & \multicolumn{1}{j|}{80.67} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{base}$ & \multicolumn{1}{j|}{34.69} & \multicolumn{1}{j|}{\textbf{34.69}} & \multicolumn{1}{j|}{\textbf{34.69}} & \multicolumn{1}{j|}{26.39} & \multicolumn{1}{j|}{29.23} & \multicolumn{1}{j|}{27.74} & \multicolumn{1}{j|}{\textbf{95.27}} & \multicolumn{1}{j|}{73.83} & \multicolumn{1}{j|}{83.19} & \multicolumn{1}{j|}{88.27} & \multicolumn{1}{j|}{80.91} & \multicolumn{1}{j|}{84.43} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{large}$ & \multicolumn{1}{j|}{27.78} & \multicolumn{1}{j|}{25.51} & \multicolumn{1}{j|}{26.60} & \multicolumn{1}{j|}{25.90} & \multicolumn{1}{j|}{27.69} & \multicolumn{1}{j|}{26.77} & \multicolumn{1}{j|}{94.59} & \multicolumn{1}{j|}{64.78} & \multicolumn{1}{j|}{76.90} & \multicolumn{1}{j|}{91.35} & \multicolumn{1}{j|}{80.27} & \multicolumn{1}{j|}{85.45} \\ \cline{2-15} 
 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Join Span\\ Detection\\ \& Labeling\end{tabular}}} & $\text{XLM-R}_\text{base}$ & \multicolumn{1}{j|}{10.90} & \multicolumn{1}{j|}{17.35} & \multicolumn{1}{j|}{13.39} & \multicolumn{1}{j|}{7.81} & \multicolumn{1}{j|}{14.12} & \multicolumn{1}{j|}{10.05} & \multicolumn{1}{j|}{91.86} & \multicolumn{1}{j|}{76.15} & \multicolumn{1}{j|}{83.27} & \multicolumn{1}{j|}{91.75} & \multicolumn{1}{j|}{76.72} & \multicolumn{1}{j|}{83.57} \\ \cline{3-15} 
 &  & $\text{XLM-R}_\text{large}$ & \multicolumn{1}{j|}{4.46} & \multicolumn{1}{j|}{10.20} & \multicolumn{1}{j|}{6.21} & \multicolumn{1}{j|}{4.62} & \multicolumn{1}{j|}{11.45} & \multicolumn{1}{j|}{6.58} & \multicolumn{1}{j|}{87.94} & \multicolumn{1}{j|}{74.89} & \multicolumn{1}{j|}{80.89} & \multicolumn{1}{j|}{77.19} & \multicolumn{1}{j|}{82.81} & \multicolumn{1}{j|}{79.90} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{base}$ & \multicolumn{1}{j|}{12.82} & \multicolumn{1}{j|}{20.41} & \multicolumn{1}{j|}{15.75} & \multicolumn{1}{j|}{8.12} & \multicolumn{1}{j|}{16.79} & \multicolumn{1}{j|}{10.95} & \multicolumn{1}{j|}{97.33} & \multicolumn{1}{j|}{70.91} & \multicolumn{1}{j|}{82.04} & \multicolumn{1}{j|}{89.75} & \multicolumn{1}{j|}{78.27} & \multicolumn{1}{j|}{83.62} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{large}$ & \multicolumn{1}{j|}{12.88} & \multicolumn{1}{j|}{17.35} & \multicolumn{1}{j|}{14.78} & \multicolumn{1}{j|}{7.71} & \multicolumn{1}{j|}{14.89} & \multicolumn{1}{j|}{10.16} & \multicolumn{1}{j|}{89.66} & \multicolumn{1}{j|}{64.22} & \multicolumn{1}{j|}{74.83} & \multicolumn{1}{j|}{91.49} & \multicolumn{1}{j|}{77.06} & \multicolumn{1}{j|}{83.66} \\ \hline
\multirow{8}{*}{\textbf{CRF}} & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Unlabeled\\ Span\\ Detection\end{tabular}}} & $\text{XLM-R}_\text{base}$ & \multicolumn{1}{j|}{30.61} & \multicolumn{1}{j|}{30.61} & \multicolumn{1}{j|}{30.61} & \multicolumn{1}{j|}{\textbf{32.54}} & \multicolumn{1}{j|}{31.54} & \multicolumn{1}{j|}{32.03} & \multicolumn{1}{j|}{88.57} & \multicolumn{1}{j|}{\textbf{82.10}} & \multicolumn{1}{j|}{85.21} & \multicolumn{1}{j|}{87.42} & \multicolumn{1}{j|}{82.51} & \multicolumn{1}{j|}{84.90} \\ \cline{3-15} 
 &  & $\text{XLM-R}_\text{large}$ & \multicolumn{1}{j|}{29.41} & \multicolumn{1}{j|}{30.61} & \multicolumn{1}{j|}{30.00} & \multicolumn{1}{j|}{26.21} & \multicolumn{1}{j|}{29.23} & \multicolumn{1}{j|}{27.64} & \multicolumn{1}{j|}{84.23} & \multicolumn{1}{j|}{72.19} & \multicolumn{1}{j|}{77.74} & \multicolumn{1}{j|}{76.81} & \multicolumn{1}{j|}{\textbf{83.12}} & \multicolumn{1}{j|}{79.84} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{base}$ & \multicolumn{1}{j|}{36.36} & \multicolumn{1}{j|}{32.65} & \multicolumn{1}{j|}{34.41} & \multicolumn{1}{j|}{32.33} & \multicolumn{1}{j|}{\textbf{33.08}} & \multicolumn{1}{j|}{\textcolor{red}{\textbf{32.70}}} & \multicolumn{1}{j|}{97.38} & \multicolumn{1}{j|}{73.65} & \multicolumn{1}{j|}{83.87} & \multicolumn{1}{j|}{87.62} & \multicolumn{1}{j|}{82.29} & \multicolumn{1}{j|}{84.87} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{large}$ & \multicolumn{1}{j|}{36.25} & \multicolumn{1}{j|}{29.59} & \multicolumn{1}{j|}{32.58} & \multicolumn{1}{j|}{31.78} & \multicolumn{1}{j|}{28.85} & \multicolumn{1}{j|}{30.24} & \multicolumn{1}{j|}{91.93} & \multicolumn{1}{j|}{68.20} & \multicolumn{1}{j|}{78.31} & \multicolumn{1}{j|}{\textbf{92.72}} & \multicolumn{1}{j|}{80.20} & \multicolumn{1}{j|}{\textcolor{red}{\textbf{86.00}}} \\ \cline{2-15} 
 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Join Span\\ Detection\\ \& Labeling\end{tabular}}} & $\text{XLM-R}_\text{base}$ & \multicolumn{1}{j|}{29.00} & \multicolumn{1}{j|}{29.59} & \multicolumn{1}{j|}{29.29} & \multicolumn{1}{j|}{26.64} & \multicolumn{1}{j|}{27.86} & \multicolumn{1}{j|}{27.24} & \multicolumn{1}{j|}{93.02} & \multicolumn{1}{j|}{78.73} & \multicolumn{1}{j|}{\textbf{85.28}} & \multicolumn{1}{j|}{88.75} & \multicolumn{1}{j|}{80.10} & \multicolumn{1}{j|}{84.20} \\ \cline{3-15} 
 &  & $\text{XLM-R}_\text{large}$ & \multicolumn{1}{j|}{27.08} & \multicolumn{1}{j|}{26.53} & \multicolumn{1}{j|}{26.80} & \multicolumn{1}{j|}{23.59} & \multicolumn{1}{j|}{25.57} & \multicolumn{1}{j|}{24.54} & \multicolumn{1}{j|}{93.33} & \multicolumn{1}{j|}{67.48} & \multicolumn{1}{j|}{78.33} & \multicolumn{1}{j|}{87.23} & \multicolumn{1}{j|}{77.12} & \multicolumn{1}{j|}{81.86} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{base}$ & \multicolumn{1}{j|}{28.12} & \multicolumn{1}{j|}{27.55} & \multicolumn{1}{j|}{27.84} & \multicolumn{1}{j|}{24.50} & \multicolumn{1}{j|}{27.86} & \multicolumn{1}{j|}{26.07} & \multicolumn{1}{j|}{94.89} & \multicolumn{1}{j|}{69.50} & \multicolumn{1}{j|}{80.24} & \multicolumn{1}{j|}{89.44} & \multicolumn{1}{j|}{80.61} & \multicolumn{1}{j|}{84.80} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{large}$ & \multicolumn{1}{j|}{\textbf{37.80}} & \multicolumn{1}{j|}{31.63} & \multicolumn{1}{j|}{34.44} & \multicolumn{1}{j|}{28.40} & \multicolumn{1}{j|}{27.10} & \multicolumn{1}{j|}{27.73} & \multicolumn{1}{j|}{92.63} & \multicolumn{1}{j|}{68.72} & \multicolumn{1}{j|}{78.91} & \multicolumn{1}{j|}{92.40} & \multicolumn{1}{j|}{79.19} & \multicolumn{1}{j|}{85.28} \\ \hline
\end{tabular}%
}
\caption{Unlabeled abusive span detection performances on dev and test sets}
\label{tab:mainres:1}
\end{table*}}

{\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|l|llllll|llllll|}
\hline
\multirow{3}{*}{\rotatebox{90}{\small{\textbf{Decoder~}}}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Training\\ Strategy\end{tabular}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Pre-trained\\ Language\\ Model\end{tabular}}}} & \multicolumn{6}{c|}{\textbf{Strict}} & \multicolumn{6}{c|}{\textbf{Relaxed}} \\ \cline{4-15} 
 &  & \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\textbf{Dev}} & \multicolumn{3}{c|}{\textbf{Test}} & \multicolumn{3}{c|}{\textbf{Dev}} & \multicolumn{3}{c|}{\textbf{Test}} \\ \cline{4-15} 
 &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{F}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{F}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{F}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{F}} \\ \hline
\multirow{8}{*}{\rotatebox{90}{\textbf{Softmax}}} & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Unlabeled\\ Span\\ Detection\end{tabular}}} & $\text{XLM-R}_\text{base}$ & \multicolumn{1}{j|}{22.22} & \multicolumn{1}{j|}{24.49} & \multicolumn{1}{j|}{23.30} & \multicolumn{1}{j|}{26.89} & \multicolumn{1}{j|}{27.31} & \multicolumn{1}{j|}{27.10} & \multicolumn{1}{j|}{88.00} & \multicolumn{1}{j|}{80.30} & \multicolumn{1}{j|}{83.97} & \multicolumn{1}{j|}{89.00} & \multicolumn{1}{j|}{82.96} & \multicolumn{1}{j|}{85.88} \\ \cline{3-15} 
 &  & $\text{XLM-R}_\text{large}$ & \multicolumn{1}{j|}{20.49} & \multicolumn{1}{j|}{25.51} & \multicolumn{1}{j|}{22.73} & \multicolumn{1}{j|}{24.54} & \multicolumn{1}{j|}{30.77} & \multicolumn{1}{j|}{27.30} & \multicolumn{1}{j|}{85.98} & \multicolumn{1}{j|}{73.93} & \multicolumn{1}{j|}{79.50} & \multicolumn{1}{j|}{80.54} & \multicolumn{1}{j|}{80.79} & \multicolumn{1}{j|}{80.67} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{base}$ & \multicolumn{1}{j|}{34.69} & \multicolumn{1}{j|}{\textbf{34.69}} & \multicolumn{1}{j|}{\textbf{34.69}} & \multicolumn{1}{j|}{26.39} & \multicolumn{1}{j|}{29.23} & \multicolumn{1}{j|}{27.74} & \multicolumn{1}{j|}{\textbf{95.27}} & \multicolumn{1}{j|}{73.83} & \multicolumn{1}{j|}{83.19} & \multicolumn{1}{j|}{88.27} & \multicolumn{1}{j|}{80.91} & \multicolumn{1}{j|}{84.43} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{large}$ & \multicolumn{1}{j|}{27.78} & \multicolumn{1}{j|}{25.51} & \multicolumn{1}{j|}{26.60} & \multicolumn{1}{j|}{25.90} & \multicolumn{1}{j|}{27.69} & \multicolumn{1}{j|}{26.77} & \multicolumn{1}{j|}{94.59} & \multicolumn{1}{j|}{64.78} & \multicolumn{1}{j|}{76.90} & \multicolumn{1}{j|}{91.35} & \multicolumn{1}{j|}{80.27} & \multicolumn{1}{j|}{85.45} \\ \cline{2-15} 
 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Join Span\\ Detection\\ \& Labeling\end{tabular}}} & $\text{XLM-R}_\text{base}$ & \multicolumn{1}{j|}{10.90} & \multicolumn{1}{j|}{17.35} & \multicolumn{1}{j|}{13.39} & \multicolumn{1}{j|}{7.81} & \multicolumn{1}{j|}{14.12} & \multicolumn{1}{j|}{10.05} & \multicolumn{1}{j|}{91.86} & \multicolumn{1}{j|}{76.15} & \multicolumn{1}{j|}{83.27} & \multicolumn{1}{j|}{91.75} & \multicolumn{1}{j|}{76.72} & \multicolumn{1}{j|}{83.57} \\ \cline{3-15} 
 &  & $\text{XLM-R}_\text{large}$ & \multicolumn{1}{j|}{4.46} & \multicolumn{1}{j|}{10.20} & \multicolumn{1}{j|}{6.21} & \multicolumn{1}{j|}{4.62} & \multicolumn{1}{j|}{11.45} & \multicolumn{1}{j|}{6.58} & \multicolumn{1}{j|}{87.94} & \multicolumn{1}{j|}{74.89} & \multicolumn{1}{j|}{80.89} & \multicolumn{1}{j|}{77.19} & \multicolumn{1}{j|}{82.81} & \multicolumn{1}{j|}{79.90} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{base}$ & \multicolumn{1}{j|}{12.82} & \multicolumn{1}{j|}{20.41} & \multicolumn{1}{j|}{15.75} & \multicolumn{1}{j|}{8.12} & \multicolumn{1}{j|}{16.79} & \multicolumn{1}{j|}{10.95} & \multicolumn{1}{j|}{97.33} & \multicolumn{1}{j|}{70.91} & \multicolumn{1}{j|}{82.04} & \multicolumn{1}{j|}{89.75} & \multicolumn{1}{j|}{78.27} & \multicolumn{1}{j|}{83.62} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{large}$ & \multicolumn{1}{j|}{12.88} & \multicolumn{1}{j|}{17.35} & \multicolumn{1}{j|}{14.78} & \multicolumn{1}{j|}{7.71} & \multicolumn{1}{j|}{14.89} & \multicolumn{1}{j|}{10.16} & \multicolumn{1}{j|}{89.66} & \multicolumn{1}{j|}{64.22} & \multicolumn{1}{j|}{74.83} & \multicolumn{1}{j|}{91.49} & \multicolumn{1}{j|}{77.06} & \multicolumn{1}{j|}{83.66} \\ \hline
\multirow{8}{*}{\rotatebox{90}{\textbf{CRF}}} & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Unlabeled\\ Span\\ Detection\end{tabular}}} & $\text{XLM-R}_\text{base}$ & \multicolumn{1}{j|}{30.61} & \multicolumn{1}{j|}{30.61} & \multicolumn{1}{j|}{30.61} & \multicolumn{1}{j|}{\textbf{32.54}} & \multicolumn{1}{j|}{31.54} & \multicolumn{1}{j|}{32.03} & \multicolumn{1}{j|}{88.57} & \multicolumn{1}{j|}{\textbf{82.10}} & \multicolumn{1}{j|}{85.21} & \multicolumn{1}{j|}{87.42} & \multicolumn{1}{j|}{82.51} & \multicolumn{1}{j|}{84.90} \\ \cline{3-15} 
 &  & $\text{XLM-R}_\text{large}$ & \multicolumn{1}{j|}{29.41} & \multicolumn{1}{j|}{30.61} & \multicolumn{1}{j|}{30.00} & \multicolumn{1}{j|}{26.21} & \multicolumn{1}{j|}{29.23} & \multicolumn{1}{j|}{27.64} & \multicolumn{1}{j|}{84.23} & \multicolumn{1}{j|}{72.19} & \multicolumn{1}{j|}{77.74} & \multicolumn{1}{j|}{76.81} & \multicolumn{1}{j|}{\textbf{83.12}} & \multicolumn{1}{j|}{79.84} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{base}$ & \multicolumn{1}{j|}{36.36} & \multicolumn{1}{j|}{32.65} & \multicolumn{1}{j|}{34.41} & \multicolumn{1}{j|}{32.33} & \multicolumn{1}{j|}{\textbf{33.08}} & \multicolumn{1}{j|}{\textcolor{red}{\textbf{32.70}}} & \multicolumn{1}{j|}{97.38} & \multicolumn{1}{j|}{73.65} & \multicolumn{1}{j|}{83.87} & \multicolumn{1}{j|}{87.62} & \multicolumn{1}{j|}{82.29} & \multicolumn{1}{j|}{84.87} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{large}$ & \multicolumn{1}{j|}{36.25} & \multicolumn{1}{j|}{29.59} & \multicolumn{1}{j|}{32.58} & \multicolumn{1}{j|}{31.78} & \multicolumn{1}{j|}{28.85} & \multicolumn{1}{j|}{30.24} & \multicolumn{1}{j|}{91.93} & \multicolumn{1}{j|}{68.20} & \multicolumn{1}{j|}{78.31} & \multicolumn{1}{j|}{\textbf{92.72}} & \multicolumn{1}{j|}{80.20} & \multicolumn{1}{j|}{\textcolor{red}{\textbf{86.00}}} \\ \cline{2-15} 
 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Join Span\\ Detection\\ \& Labeling\end{tabular}}} & $\text{XLM-R}_\text{base}$ & \multicolumn{1}{j|}{29.00} & \multicolumn{1}{j|}{29.59} & \multicolumn{1}{j|}{29.29} & \multicolumn{1}{j|}{26.64} & \multicolumn{1}{j|}{27.86} & \multicolumn{1}{j|}{27.24} & \multicolumn{1}{j|}{93.02} & \multicolumn{1}{j|}{78.73} & \multicolumn{1}{j|}{\textbf{85.28}} & \multicolumn{1}{j|}{88.75} & \multicolumn{1}{j|}{80.10} & \multicolumn{1}{j|}{84.20} \\ \cline{3-15} 
 &  & $\text{XLM-R}_\text{large}$ & \multicolumn{1}{j|}{27.08} & \multicolumn{1}{j|}{26.53} & \multicolumn{1}{j|}{26.80} & \multicolumn{1}{j|}{23.59} & \multicolumn{1}{j|}{25.57} & \multicolumn{1}{j|}{24.54} & \multicolumn{1}{j|}{93.33} & \multicolumn{1}{j|}{67.48} & \multicolumn{1}{j|}{78.33} & \multicolumn{1}{j|}{87.23} & \multicolumn{1}{j|}{77.12} & \multicolumn{1}{j|}{81.86} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{base}$ & \multicolumn{1}{j|}{28.12} & \multicolumn{1}{j|}{27.55} & \multicolumn{1}{j|}{27.84} & \multicolumn{1}{j|}{24.50} & \multicolumn{1}{j|}{27.86} & \multicolumn{1}{j|}{26.07} & \multicolumn{1}{j|}{94.89} & \multicolumn{1}{j|}{69.50} & \multicolumn{1}{j|}{80.24} & \multicolumn{1}{j|}{89.44} & \multicolumn{1}{j|}{80.61} & \multicolumn{1}{j|}{84.80} \\ \cline{3-15} 
 &  & $\text{PhoBERT}_\text{large}$ & \multicolumn{1}{j|}{\textbf{37.80}} & \multicolumn{1}{j|}{31.63} & \multicolumn{1}{j|}{34.44} & \multicolumn{1}{j|}{28.40} & \multicolumn{1}{j|}{27.10} & \multicolumn{1}{j|}{27.73} & \multicolumn{1}{j|}{92.63} & \multicolumn{1}{j|}{68.72} & \multicolumn{1}{j|}{78.91} & \multicolumn{1}{j|}{92.40} & \multicolumn{1}{j|}{79.19} & \multicolumn{1}{j|}{85.28} \\ \hline
\end{tabular}%
}
\caption{Unlabeled abusive span detection performances on dev and test sets}
\label{tab:mainres:1}
\end{table*}}



==> tabs/mainres_2.tex <==
% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|c|l|ccccccc|ccccccc|}
% \hline
% \multirow{2}{*}{\rotatebox{90}{\textbf{Decoder~}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Pre-trained\\ Language\\ Model\end{tabular}}}} & \multicolumn{7}{c|}{\textbf{Strict}} & \multicolumn{7}{c|}{\textbf{Relaxed}} \\ \cline{3-16} 
%  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Cultural Identity~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Financial Economic~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Mental Psychological~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Physical~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Sexual~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Verbal Emotional~}}} & \rotatebox{90}{\textbf{Overall~}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Cultural Identity~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Financial Economic~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Mental Psychological~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Physical~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Sexual~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Verbal Emotional~}}} & \rotatebox{90}{\textbf{Overall~}} \\ \hline
% \multirow{4}{*}{\rotatebox{90}{\textbf{Softmax}}} & $\text{XLM-R}_\text{base}$ & \multicolumn{1}{c|}{00.01} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 \\ \cline{2-16} 
%  & $\text{XLM-R}_\text{large}$ & \multicolumn{1}{c|}{00.02} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 \\ \cline{2-16} 
%  & $\text{PhoBERT}_\text{base}$ & \multicolumn{1}{c|}{00.03} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 \\ \cline{2-16} 
%  & $\text{PhoBERT}_\text{large}$ & \multicolumn{1}{c|}{00.04} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 \\ \hline
% \multirow{4}{*}{\rotatebox{90}{\textbf{CRF}}} & $\text{XLM-R}_\text{base}$ & \multicolumn{1}{c|}{00.05} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 \\ \cline{2-16} 
%  & $\text{XLM-R}_\text{large}$ & \multicolumn{1}{c|}{00.06} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 \\ \cline{2-16} 
%  & $\text{PhoBERT}_\text{base}$ & \multicolumn{1}{c|}{00.07} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 \\ \cline{2-16} 
%  & $\text{PhoBERT}_\text{large}$ & \multicolumn{1}{c|}{00.08} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & \multicolumn{1}{c|}{00.00} & 00.00 \\ \hline
% \end{tabular}%
% }
% \caption{Labeled abusive span detection F-scores on test set of models using join span detection and labeling training strategy}
% \label{tab:mainres:2}
% \end{table*}


\begin{table*}[t]
\centering
\caption{Labeled abusive span detection F-scores on test set of models using join span detection and labeling training strategy}
\label{tab:mainres:2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|l|ccccccc|ccccccc|}
\hline
\multirow{2}{*}{\rotatebox{90}{\textbf{Decoder~}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Pre-trained\\ Language\\ Model\end{tabular}}}} & \multicolumn{7}{c|}{\textbf{Strict}} & \multicolumn{7}{c|}{\textbf{Relaxed}} \\ \cline{3-16} 
 & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Cultural Identity~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Financial Economic~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Mental Psychological~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Physical~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Sexual~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Verbal Emotional~}}} & \rotatebox{90}{\textbf{Overall~}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Cultural Identity~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Financial Economic~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Mental Psychological~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Physical~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Sexual~}}} & \multicolumn{1}{c|}{\rotatebox{90}{\textbf{Verbal Emotional~}}} & \rotatebox{90}{\textbf{Overall~}} \\ \hline
\multirow{4}{*}{\rotatebox{90}{\textbf{Softmax}}} & $\text{XLM-R}_\text{base}$ & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{9.09} & \multicolumn{1}{j|}{5.88} & \multicolumn{1}{j|}{8.62} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{12.40} & \multicolumn{1}{j|}{8.15} & \multicolumn{1}{j|}{28.43} & \multicolumn{1}{j|}{\textbf{66.58}} & \multicolumn{1}{j|}{46.88} & \multicolumn{1}{j|}{59.05} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{64.55} & \multicolumn{1}{j|}{55.41} \\ \cline{2-16} 
 & $\text{XLM-R}_\text{large}$ & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{1.96} & \multicolumn{1}{j|}{4.40} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{5.71} & \multicolumn{1}{j|}{4.17} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{48.43} & \multicolumn{1}{j|}{42.68} & \multicolumn{1}{j|}{26.71} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{51.92} & \multicolumn{1}{j|}{44.43} \\ \cline{2-16} 
 & $\text{PhoBERT}_\text{base}$ & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{9.26} & \multicolumn{1}{j|}{7.48} & \multicolumn{1}{j|}{5.66} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{11.28} & \multicolumn{1}{j|}{8.46} & \multicolumn{1}{j|}{11.89} & \multicolumn{1}{j|}{60.84} & \multicolumn{1}{j|}{55.01} & \multicolumn{1}{j|}{44.66} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{63.10} & \multicolumn{1}{j|}{55.70} \\ \cline{2-16} 
 & $\text{PhoBERT}_\text{large}$ & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{1.79} & \multicolumn{1}{j|}{8.89} & \multicolumn{1}{j|}{2.13} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{10.37} & \multicolumn{1}{j|}{7.29} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{64.21} & \multicolumn{1}{j|}{54.51} & \multicolumn{1}{j|}{38.10} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{61.50} & \multicolumn{1}{j|}{54.55} \\ \hline
\multirow{4}{*}{\rotatebox{90}{\textbf{CRF}}} & $\text{XLM-R}_\text{base}$ & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{12.90} & \multicolumn{1}{j|}{18.27} & \multicolumn{1}{j|}{8.82} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{\textbf{27.06}} & \multicolumn{1}{j|}{18.28} & \multicolumn{1}{j|}{\textbf{38.86}} & \multicolumn{1}{j|}{65.10} & \multicolumn{1}{j|}{51.34} & \multicolumn{1}{j|}{27.12} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{\textbf{70.82}} & \multicolumn{1}{j|}{55.41} \\ \cline{2-16} 
 & $\text{XLM-R}_\text{large}$ & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{\textbf{17.86}} & \multicolumn{1}{j|}{15.38} & \multicolumn{1}{j|}{\textbf{25.00}} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{15.05} & \multicolumn{1}{j|}{16.48} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{58.52} & \multicolumn{1}{j|}{49.36} & \multicolumn{1}{j|}{\textbf{61.03}} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{53.96} & \multicolumn{1}{j|}{51.84} \\ \cline{2-16} 
 & $\text{PhoBERT}_\text{base}$ & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{15.62} & \multicolumn{1}{j|}{17.53} & \multicolumn{1}{j|}{19.44} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{20.59} & \multicolumn{1}{j|}{17.86} & \multicolumn{1}{j|}{26.11} & \multicolumn{1}{j|}{66.50} & \multicolumn{1}{j|}{54.20} & \multicolumn{1}{j|}{58.27} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{61.18} & \multicolumn{1}{j|}{57.46} \\ \cline{2-16} 
 & $\text{PhoBERT}_\text{large}$ & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{17.24} & \multicolumn{1}{j|}{\textbf{18.95}} & \multicolumn{1}{j|}{20.00} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{21.95} & \multicolumn{1}{j|}{\textcolor{red}{\textbf{18.75}}} & \multicolumn{1}{j|}{29.24} & \multicolumn{1}{j|}{61.65} & \multicolumn{1}{j|}{\textbf{58.36}} & \multicolumn{1}{j|}{54.11} & \multicolumn{1}{j|}{0.00} & \multicolumn{1}{j|}{64.44} & \multicolumn{1}{j|}{\textcolor{red}{\textbf{58.10}}} \\ \hline
\end{tabular}%
}
\end{table*}
